The nature of sub-millimeter and highly star-forming galaxies in the EAGLE simulation

We exploit EAGLE, a cosmological hydrodynamical simulation, to reproduce the selection of the observed sub-millimeter (submm) galaxy population by selecting the model galaxies at $z \geq 1$ with mock submm fluxes $S_{850} \geq 1$ mJy. There is a reasonable agreement between the galaxies within this sample and the properties of the observed submm population, such as their star formation rates (SFRs) at $z<3$, redshift distribution and many integrated galaxy properties. We find that the bulk of the $S_{850} \geq 1$ mJy model population is at $z = 2.5$, and that they are massive galaxies ($M_* \sim 10^{11}$ Msol) with high dust masses ($M_{\mathrm{dust}} \sim 10^{8}$ Msol), gas fractions ($f_{\mathrm{gas}} \approx 50$%) and SFRs ($\dot M_* \approx 100$ Msol/yr). They have major and minor merger fractions similar to the general population, suggesting that mergers are not the primary driver of the model submm galaxies. Instead, the $S_{850} \geq 1$ mJy model galaxies yield high SFRs primarily because they maintain a significant gas reservoir as a result of hosting an undermassive black hole. In addition, we find that not all highly star-forming EAGLE galaxies have submm fluxes $S_{850} > 1$ mJy. Thus, we investigate the nature of $z \geq 1$ highly star-forming Submm-Faint galaxies (i.e., $\dot M_* \geq 80$ Msol/yr but $S_{850}< 1$ mJy). We find they are similar to the model submm galaxies; being gas rich and hosting undermassive black holes, however they are typically lower mass ($M_* \sim 10^{10}$ Msol) and are at higher redshifts ($z>4$). These typically higher-$z$ galaxies show stronger evidence for having been triggered by major mergers, and critically, they are likely missed by current submm surveys due to their higher dust temperatures. This suggests a potentially even larger contribution to the SFR density at $z > 3$ from dust-obscured systems than implied by current observations.

==> extras.tex <==

\begin{enumerate}

\item Compute the volume number density (d$N$/d$V$) of \smmbright galaxies at each snapshot.
\item Assume this volume number density holds for a small interval in redshift, $\Delta z = 0.05$, centred on the redshift of the snapshot.
\item Linearly interpolate the values of d$N$/d$V$d$z$ between the snapshots in intervals of $\Delta z = 0.05$.
\item Integrate over all redshift intervals ($1<z<20$) and their associated comoving volumes to obtain the \emph{total} number of \smmbright galaxies within the model universe.
\item Divide by the area of the entire sky.

\end{enumerate}

\subsection{The submillimeter properties of strongly star-forming galaxies}
\label{sect:smm}

Current surveys in the far-infrared and \smm consistently report galaxy populations at $z \gtrsim 1$ with space densities of $\sim 10^{-4}$--$10^{-5}$ cMpc$^{-3}$ and inferred SFRs in excess of 100~\Msolyr, which would easily meet our strongly star forming criteria. We now wish to compare the \eagle strongly star-forming galaxies with these observations. We note, for this section we transition to using the strongly star-forming sample produced by the snapshot output (see \cref{sect:sim_output}), as the radiative transfer post-processing is only computed for the model galaxies at these times (see \cref{sect:radiative_transfer}).

We define the model galaxies with \fsmm greater than 1~mJy to be \squotes{\smmbright} and those with \fsmm less than 1~mJy to be \squotes{\smmfaint}. This cut broadly reflects the definitions in the literature for strongly star-forming sources derived from the observations \citep[e.g.,][]{Simpson2014,Cowie2018}. Perhaps surprisingly, we find that the majority of the model galaxies within the strongly star-forming sample are \smmfaint (89/129, 69\%), as opposed to \smmbright (40/129, 31\%). \cref{fig:z_dist} shows the redshift distributions of the galaxies within the \smmbright and \smmfaint subsets. Interestingly, whilst all these model galaxies are strongly star-forming, those that are \smmbright preferentially exist at intermediate redshifts ($z \approx 2$) and those
that are \smmfaint preferentially exist at higher redshifts ($z \approx 5$). 

As the strongly star-forming \smmfaint galaxies within our sample would likely not be detected by current \smm surveys, we only compare directly to the \smmbright subset in the next section. We return to the properties of the \smmfaint strongly star-forming galaxies, and what differentiates them from the galaxies within the \smmbright subset, in \cref{sect:smm_bright_faint_diff}. 

\subsubsection{A comparison to the observed submillimeter population}
\label{sect:observations_smm}

\section{The \eagle simulation}
\label{sect:eagle}

The \dquotes{Evolution and Assembly of GaLaxies and their Environment}
\citep[\eagle,][]{Schaye2015,Crain2015} \footnote{\url{www.eaglesim.org}}\textsuperscript{,}\footnote{Galaxy and halo catalogues of the simulation suite, as well as the particle data, are publicly available at \url{http://www.eaglesim.org/database.php} \citep{McAlpine2015,EAGLE2017}.} is a suite of hydrodynamical cosmological simulations that cover a wide range of periodic volumes, numerical resolutions and physical models. To incorporate the processes that operate below the simulation resolution a series of \squotes{subgrid} prescriptions are implemented, namely: radiative cooling and photo-ionisation heating \citep{Wiersma2009a}; star formation \citep{Schaye2008}, stellar mass loss \citep{Wiersma2009b} and stellar feedback \citep{DallaVecchia_Schaye2012}; black hole growth via accretion and mergers and black hole feedback \citep{Springel2005a,RosasGuevara2016}. The free parameters in these models are calibrated to reproduce the observed galaxy stellar mass function, galaxy sizes and normalization of the black hole mass--bulge mass relation at $z \approx 0.1$.  A full description of the simulation and the calibration strategy can be found in \citet{Schaye2015} and \citet{Crain2015}, respectively. 

For this study we are interested in the most strongly star-forming galaxies ($\dot M_{*} \geq 80$ \Msolyr), and therefore restrict our study to the largest simulation, Ref-L0100N1504, which contains the greatest number of these objects.  This simulation is a cubic periodic volume 100 comoving megaparsecs (cMpc) on each side, containing $1504^{3}$ dark matter particles of mass $9.7 \times 10^{6}$~\Msol and an equal number of baryonic particles with an initial mass of $1.8 \times 10^{6}$~\Msol.  The subgrid parameters are those of the \eagle reference model, described fully by \citet{Schaye2015}. The simulation adopts a flat $\Lambda$CDM cosmogony with parameters inferred from analysis of {\it Planck} data \citep{Planck2013}: $\Omega_\Lambda = $\,0.693, $\Omega_{\rm m} = $\,0.307, $\Omega_{\rm b} =$\,0.048, $\sigma_8 =$\,0.8288, $n_{\rm s} = $\,0.9611 and $H_0 = $\,67.77\,km\,s$^{-1}$\,Mpc$^{-1}$. A \citet{Chabrier2003} stellar initial mass function (IMF) is also adopted.  

\subsection{Simulation output}
\label{sect:sim_output}

To produce a galaxy catalog, the substructure finding algorithm \subfind \citep{Springel2001,Dolag2009} is applied to the 29 \squotes{snapshot} outputs and 200 of the data-lite \squotes{snipshot} outputs between redshifts $z=20$ and $z=0$. These store the current state of the simulation at the given time, and have temporal spacings of $\approx$ 400--800~Myr and $\approx$ 40--80~Myr, respectively.

Halo mass, \M{200}, is defined as the total mass enclosed within $r_{\mathrm{200}}$, the radius at which the mean enclosed density is 200 times the critical density of the Universe. Galaxy mass, \M{*}, is defined as the total stellar content bound to a subhalo within a spherical aperture with radius 30~proper kiloparsecs (pkpc), as per \citet{Schaye2015}. The sizes of galaxies are quoted in physical units, unless stated otherwise.

\subsubsection{Merger trees}

The histories of galaxies are tracked using a merger tree (independently performed on the snapshot and snipshot output). As the hierarchical build-up of galaxies can be complex, the history of each galaxy is considered from the reference frame of their \squotes{main progenitor}, the branch of the galaxy's full merger tree that contains the greatest total mass \citep[see][ for full details]{Qu2017}.

The completion time of a galaxy--galaxy merger is defined as the cosmic time of the first simulation output where two galaxies that were previously identified as separate individually bound objects are now identified as a single bound object by the \subfind algorithm. Mergers are classified by their stellar mass ratio,  $\mu = M_{*,1} / M_{*,2}$, where $M_{*,2}$ is the mass of the most massive member of the binary. They are considered major if $\mu \geq \frac{1}{4}$, minor if $\frac{1}{10} \leq \mu < \frac{1}{4}$ and either major or minor if $\mu \geq \frac{1}{10}$. To account for the stellar stripping that occurs during the later stages of the interaction, the stellar mass ratio is computed when the in-falling galaxy had its maximum mass \citep[e.g.,][]{Rodriguez-Gomez2015,Qu2017}. Additionally, mergers are only considered \squotes{resolved} when $M_{*,2} \geq 10^{8}$ \Msol ($\approx 100$ stellar particles).

\subsubsection{Mock observables}
\label{sect:radiative_transfer}

The light observed from a galaxy is a combination of intrinsic and scattered light. Therefore to accurately compare the observables of model galaxies to the observations we are required to solve the complete three-dimensional radiative transfer problem. For \eagle, this is performed in post-processing using information from the star-forming regions, stellar sources, and the diffuse dust distribution of the model galaxies using the radiative transfer code {\sc skirt} \citep{Baes2011,Camps2015}. This produces mock observables for the model galaxies from the ultraviolet to the submillimeter (\smm) wavebands\footnote{The rest-frame magnitudes and observer-frame fluxes for all \eagle galaxies with stellar masses greater than $10^{8.5}$ \Msol are publicly available \citep{Camps2018}.}. The radiative transfer post processing is only performed for the model galaxies within the 29 snapshot outputs.

For the analysis in \cref{sect:smm} we compare to the observed \smm population using the {\sc skirt} inferred observed-frame fluxes at 850$\mu$m \citep[\fsmm, column {\sc SCUBA2\_850} in the public database,][]{McAlpine2015,Camps2018}.

\subsection{Selecting strongly star-forming model galaxies}
\label{sect:smg_selection}

We wish to use \eagle to study the properties of the most strongly star-forming galaxies ($\dot M_{*} \gtrsim 100$ \Msolyr). For this we apply a selection to isolate the most strongly star-forming galaxies, adopting a space density which is representative of the limits on strongly star-forming populations derived from a variety of observational techniques. We take this approach as the various observational techniques used to estimate the space density of strongly star-forming galaxies at $z>1$ suffer from a range of biases or shortcomings. For example, wide-field, narrow-band H$\alpha$ surveys estimate space densities of $\sim 10^{-4}$ cMpc$^{-3}$ at $z\geq 1.5$ \citep{Sobral2013}, however, many of these bright H$\alpha$ sources are AGN \citep{Sobral2016}, while narrower field spectroscopic and grism surveys sample much smaller volumes and the grism surveys do not cover H$\alpha$ beyond $z\approx 1.5$ \citep[e.g.,][]{Atek2010,Brammer2012,Pirzkal2013}.  Equally, surveys which select sources on the basis of their mid- or far-infrared luminosity (as a proxy for their SFR) have reported space densities of $\sim 2 \times 10^{-4}$--$10^{-5}$ cMpc$^{-3}$ for galaxies with far-infrared luminosities of $\gtrsim 10^{12}$ L$_\odot$ and inferred SFRs of $\gtrsim 100$ \Msolyr at $z\approx$ 1.5--2.5 \citep[e.g.,][]{Chapman2005,Magnelli2011,Casey2012,Gruppioni2013,Swinbank2014,Koprowski2017}.  Again, these studies suffer from a combination of AGN contamination of the derived luminosities \citep[a particular problem in the mid-infrared, e.g.,][]{Kirkpatrick2012,Kirkpatrick2015,DelMoro2013}, or blending and misidentification of the correct galaxy counterparts in low-resolution far-infrared and sub-millimeter surveys \citep[e.g.,][]{Hodge2013,Casey2014,Simpson2014}.

ALMA is starting to address some of these concerns, but has so far only undertaken surveys at sub-/millimeter wavelengths and therefore selects sources on a combination of dust temperature and far-infrared luminosity, rather than purely on the SFR.  Nevertheless, current sub-/millimeter studies of blank fields, as well as follow-ups of wide-field single-dish sub-millimeter surveys yields space densities of $\sim 1$--5 $\times 10^{-5}$ cMpc$^{-3}$ at equivalent 870~$\mu$m fluxes of 1--4~mJy, equivalent to inferred SFRs of 70--300 \Msolyr \citep[e.g.,][]{Swinbank2014,Aravena2016,Walter2016,Dunlop2017,Stach2018}. Given the reliability of the identification of the counterparts to the sub-/millimeter sources provided by ALMA's sub-arcsecond spatial resolution, we will use these samples later in our comparison to the predicted properties from \eagle. 

Given the range and uncertainties in the various estimates of the space density for strongly star-forming galaxies from the observations, we have chosen to select an equivalent SFR limit which roughly corresponds to the space densities derived from the observations, $\sim 2 \times 10^{-4}$--$10^{-5}$ cMpc$^{-3}$, and which allows us to isolate a sufficient sample ($\gtrsim 100$ galaxies) of strongly star-forming galaxies to allow for a statistical analysis (see \cref{fig:volume_density}). Our adopted SFR limit is $\geq 80$ \Msolyr, which corresponds to a typical space density of star-forming galaxies in \eagle of $8 \times 10^{-5}$ cMpc$^{-3}$ (indicated in \cref{fig:volume_density}). Nevertheless, as we show in \cref{sect:smm}, the predicted properties of these strongly star-forming model galaxies are reasonably well-matched to the multiwavelength properties of the observed populations, supporting their use to address the questions which the observations either have difficulty answering, or cannot answer (e.g., triggering, evolutionary connections, etc).

We construct two samples: those galaxies that are identified to be strongly star-forming at the times of the snapshot output (129 galaxies) and those galaxies that are identified to be strongly star-forming at the times of the snipshot output (962 galaxies). In total, 174 \emph{unique} main-progenitor branches are identified as having hosted a strongly star-forming galaxy at least once along their history within the snipshot sample, compared to only 82 identified from the snapshot sample. The discrepancy is due to the temporal spacing of the output and their relative ability to capturing galaxies in a finite strongly star-forming phase. However, we confirm that the temporal spacing of the snipshots ($\approx$ 40--80~Myr) is sufficient to capture $>95$\% of the galaxies that were ever strongly star-forming (confirmed by the galaxy's maximum SFR derived from the stellar particles, see \cref{sect:sfr_from_particles}), giving us an almost fully complete sample of strongly star-forming galaxies in the simulation. Other than for \cref{sect:smm}, where we use the snapshot sample for the mock observable properties, the snipshot sample is used throughout this work.

\cref{fig:main_sequence} demonstrates where, relative to the star forming \squotes{main-sequence}, strongly star-forming galaxies lie in the redshift range $2 < z < 3$. We define the main-sequence as the median SFR, for a given range in stellar mass, of all \squotes{non-quenched} galaxies. For this redshift range that includes all galaxies with specific star-formation rates (sSFR $= \dot M_{*} / M_{*}$) greater than $10^{-9.6}$~yr$^{-1}$, however this value does evolve \citep[see][]{Matthee2018}. This so-called \squotes{main-sequence} is plotted on the figure. Due to its shape, strongly star-forming galaxies become increasingly offset from the main-sequence as the stellar mass decreases (up to $\approx 0.75$~dex). Additionally, as the characteristic SFR of main-sequence galaxies increases with increasing redshift \citep{Furlong2015,Matthee2018}, the offset between strongly star-forming galaxies and the main-sequence universally decreases for all stellar masses with increasing redshift.

Previous comparisons of models with observations for this galaxy population have highlighted apparent tensions with the current theory of galaxy formation \citep[e.g.,][]{Baugh2005,Swinbank2008,Dave2010,Hayward2013}.  These models generally have difficulty in matching the observed SFRs or \smm number counts while maintaining agreement with other observations of the wider galaxy population. However, the necessity of a radical solution to the discrepancy has perhaps weakened since higher resolution observational data has become available \citep[e.g.,][]{Cowley2015}.

\begin{abstract}
Far-infrared and sub-millimeter luminous galaxies are a rapidly evolving population which may make a significant contribution to the star-formation budget at $z \sim 1$.  However, the interpretation of the nature of this population is complicated by both observational limitations (e.g., the low-resolution of the surveys used to find them) and the intrinsic faintness of these galaxies at wavelengths shortward of the far-infrared wavebands, where many diagnostic features crucial for understanding the energetics and triggering of these systems are found. To aid in their interpretation, we have therefore exploited \eagle, a state-of-the-art galaxy formation simulation, to reproduce the selection of this population in the model and to understand the relationship between far-infrared luminous galaxies,  starbursts and the wider galaxy population. To this end we have implemented a simple recipe to reproduce the restframe far-infrared/sub-millimeter emission from  star-forming model galaxies in the \eagle simulation.  We discuss the properties of the population selected in terms of their observed sub-millimeter flux, compared to a sample selected to have high star-formation rates (SFR) and the bulk of the less-active galaxies.  We find that sub-millimeter and a pure SFR selection identify overlapping, but not identical samples of model galaxies.  In particular the SFR-selected sample exhibits a much higher redshift peak,  $z\sim$\,4, compared to the sub-millimeter galaxies (SMGs) whose distribution peaks at  $z\sim$\,2 (in reasonable agreement with observational constraints), both populations span a wide
range in redshift: $z\sim$\,1--6.  We find that the high-redshift end of the high-SFR sample is due to the smaller sizes of these star-forming sources which lead to higher dust temperatures, dropping them below the sub-millimeter flux limit.    For the model SMGs we find that recent major and minor mergers are much more frequent than in a  mass and redshift-matched sample of less active galaxies, suggesting that mergers do play a central role in triggering this activity in this population.  Finally, we exploit an unique aspect of theoretical simulations to trace the present-day properties of the descendants of the SMGs, finding that they evolve into typically some of the most massive galaxies at $z\sim$\,0.
\end{abstract}

Sub-millimeter galaxies (SMGs) are a population of high-redshift galaxies with high star formation rates (SFRs) and significant dust masses. The sub-millimeter emission arises from the reprocessing of the UV light from young stars by the dust \citep[see][ for a review]{Casey2014}. The SMG population are relatively rare, with a sparse number density of 10$^{-5}$\,h$^{-1}$\,Mpc$^{-3}$ at $z \approx$ 2--3 \citep[e.g.,][]{Chapman2005,Simpson2014}. However, this population remains particularly interesting due to the apparently high levels of star formation and the many open questions that remain unanswered about their formation and evolution. For example: What triggers such extreme star formation, mergers or disk instabilities? How long can these galaxies form stars at such apparently high rates? How do they evolve following the star burst episode?

Previous comparisons of models with observations for this galaxy population have highlighted apparent tensions with the current theory of galaxy formation \citep[e.g.,][]{Baugh2005,Swinbank2008,Dave2010,Hayward2013}.  These models generally have difficulty in matching the observed star formation rates or sub-millimeter number counts while maintaining agreement with other observations of the wider galaxy population. A number of solutions have been proposed for this discrepancy including ZZZ. However the necessity of a radical solution to the discrepancy has perhaps weakened since higher resolution observational data has become available \citep[e.g.,][]{Cowley2015}.


\item Lower mass ($M_{*} \lesssim 10^{11}$ \Msol) strongly star-forming galaxies at $z \gtrsim 3$ likely require a triggering merger\footnote{Although the merger fraction for these galaxies is not consistent with 100\% like their counterparts at lower redshift, their merger fractions are still high ($\approx 70$\% for $\mu \geq \frac{1}{10}$). It is also possible that lower mass ratio mergers, or mergers that are not resolved by the simulation could bring this fraction up to 100\%. We note, the merger fraction of galaxies in this redshift range and stellar mass are not enhanced relative to the main-sequence population.}. Again, the induced starburst is only maintained when the interacting galaxy is both gas rich (however this is true for all galaxies at this redshift) \emph{and} hosts an undermassive black hole (relative to galaxies on the main-sequence).

\subsubsection{An absolute calibration of star formation rates}
\label{sect:sfr_calibration}

When comparing to the observed cosmic SFR density, \citet{Furlong2015a} found an almost constant -0.2~dex offset for redshifts $z \leq 3$.  There is however continued uncertainty as to the absolute calibration of SFR indicators on which these observations rely.  For example, \citet{Chang2015} find upon revisiting this calibration with the addition of WISE photometry to the full SDSS spectroscopic galaxy sample that the SFRs of local galaxies along the
main-sequence are systematically lower than previously estimated by $\approx 0.2$~dex, yielding good agreement with the \eagle prediction \citep[see Figure 5 of][]{Schaller2015b}.

\section{A complete sampling of strongly star-forming galaxies}
\label{sect:sampling}

\begin{table}
\caption{Properties of the four strongly star-forming samples used for this study, showing, from right to left: the sample name, the total number of galaxies (unique galaxies) within the sample, the fraction that survive to the present day, the satellite fraction at the time the galaxies were strongly star-forming and the satellite fraction of the descendants at $z=0$.}
\begin{tabular}{crrrr}\hline
Sample & Num & Surviving & Sat frac & Sat frac\\
&sampled&fraction&&($z=0$)\\
\hline\hline
Snapshots & 129 (82) & 79\% & 2\% & 29\% \\
Snipshots & 962 (174) & 65\% & 2\% & 29\% \\
SMM-Bright & 40 (22) & 86\% & 5\% & 32\% \\
SMM-Faint & 89 (68) & 82\% & 2\% & 30\% \\
\hline
\end{tabular}
\label{tab:sample}
\end{table}

If the typical duration of a strongly star-forming phase is less than the temporal spacing of the simulation outputs, it is plausible that a number of galaxies undergoing a strongly star-forming phase will be missed, which would leave us with an incomplete sample. \cref{tab:sample} shows the statistics of the four strongly star-forming samples used for this study: the \textit{snapshots} sample is all the strongly star-forming galaxies sampled from the snapshots, the \textit{snipshots} sample is all the strongly star-forming galaxies sampled from the snipshots, the \textit{SMM-Bright} sample is all the strongly star-forming galaxies sampled from the snapshots with SMM fluxes $S_{850 \mu \mathrm{m}} \geq 1$~mJy and the \textit{SMM-Faint} sample is the all strongly star-forming galaxies sampled from the snapshots with SMM fluxes $S_{850 \mu \mathrm{m}} < 1$~mJy. As the same galaxies are captured to be strongly star-forming multiple times along their main progenitor branches, the number of \squotes{unique} galaxies, or more accurately the number of unique main progenitor branches, is always less than the total number of sampled events.

It is clear, that the temporal spacing of the snapshot output is not sufficient to capture all the galaxies that were once strongly star-forming; 82 unique galaxies identified, versus 174 from the snipshot sample. This leads us to ask, then, how complete the snipshot sample is at capturing all the galaxies that have ever been strongly star-forming. To check this, we compute the maximum SFR of every galaxy using their individual stellar particles. As each stellar particle records the time of its birth and its initial mass, it is possible to reconstruct a highly accurate ($\approx 1$~Myr spacing) SFR history for the entire galaxy. From this we can then obtain a complete census of all the galaxies that have ever achieved a SFR $\geq 80$ \Msolyr. \cref{fig:cumulative_fraction} shows the cumulative fraction of all the galaxies at $z=0$, as a function of the stellar mass, that have ever recorded a SFR $\geq 80$ \Msolyr in their lifetime, sampled from the snapshots, snipshots and individual stellar particle histories. It is clear from this figure, that the snipshots are indeed sufficient to capture the vast majority of strongly star-forming galaxies ($>95$\% complete).   

\begin{figure}
\includegraphics[width=\columnwidth]{plots/Cumulative_SSF_Fraction_z_0}

\caption{The cumulative fraction of all galaxies at $z=0$, as a function of the stellar mass, that were ever strongly star-forming at some point in their lifetimes (i.e., had a SFR $\geq 80$ \Msolyr). The fractions are computed separately for the snapshot sample ($\approx$ 400--800~Myr temporal spacings, blue), the snipshot sample ($\approx$ 40--80~Myr temporal spacings, orange) and from the individual stellar particle histories ($\approx$ 1-5~Myr temporal spacings, green). From this we find that the snipshot sample is sufficient to capture $>95$\% of all the galaxies that were ever strongly star-forming.} 

\label{fig:cumulative_fraction}
\end{figure}

\item The median intermediate mass strongly star-forming galaxy ($M_{*} =$ 0.2--1.0 $\times 10^{11}$ \Msol) has evolved from a galaxy that is less massive in stars (by $\approx 0.5$~dex), and less star forming (by $\approx 0.5$~dex) than the equivalent median galaxy on the main-sequence, and evolves to be more massive in stars (by $\approx 0.25$~dex) and equivalently star-forming. See \cref{fig:triggering_properties}.

\item The median intermediate mass strongly star-forming galaxy ($M_{*} =$ 0.2--1.0 $\times 10^{11}$ \Msol) has evolved from a galaxy that is hosted by a less massive halo (by $\approx 0.5$~dex), hosted a less massive black hole (by up to $\approx 2$~dex) and yielded a higher gas fraction (by up to a factor of 3) than the equivalent median galaxy on the main-sequence, and evolves to be hosted by an more massive halo (by $\approx 0.1$~dex), host a more massive black hole (by $\approx 0.25$ dex) and yield a lower gas fraction (by up to a factor of 2). See \cref{fig:triggering_properties2}.

\item The median massive strongly star-forming galaxy ($M_{*} \gtrsim 10^{11}$ \Msol) shares a very similar evolution, in terms of the SFR, stellar mass, halo mass, black hole mass and gas fraction, to the equivalent median galaxy on the main-sequence. See \cref{fig:triggering_properties}.

\item The merger rate of strongly star-forming galaxies increases with decreasing stellar mass: $56 \pm 9$\% for $M_{*} =$ 1.0--6.0 $\times 10^{11}$ \Msol increasing to $89 \pm 9$\% for $M_{*} =$ 0.2--0.5 $\times 10^{11}$ \Msol, for merger mass ratios $\mu \geq \frac{1}{10}$ in the redshift range $2 < z < 3$. The merger rate of strongly star-forming galaxies is always higher than their main-sequence counterparts; $41 \pm 8$\% and $56 \pm 2$\%, respectively, for the example above. Therefore mergers are a important component for creating strongly star-forming galaxies, particularly at lower masses. See \cref{fig:merger_fraction}.

\item The cumulative fraction of galaxies that have ever had a strongly star-forming phase in their past (i.e., have ever been above $\dot M_{*} \geq 80$ \Msolyr) decreases rapidly with decreasing stellar mass. Only $\approx 30$\% of galaxies above $M_{*} \geq 10^{11}$ \Msol have ever been previously strongly star-forming (however this fraction does evolve). Therefore a strongly star-forming phase of galaxy evolution is rare, and not ubiquitous. See \cref{fig:cumulative_fraction_evo}.   

\item The descendants of strongly star-forming galaxies at $z=0$ are among the most massive central and satellite galaxies today. The properties of the descendants are not differentiable from the median of the general population, except in the case of the black hole mass, where strongly star-forming descendants host overmassive black holes for a fixed stellar mass relative to the general population. This suggests that strong periods of stellar growth is tightly linked to strong(er) periods of black hole growth. See \cref{fig:descendant_properties}.

\item Only $\approx$ 30\% of strongly star-forming galaxies are be \squotes{Bright} at submillimeter wavelengths (\fsmm $\geq 1$~mJy). The majority of strongly star-forming galaxies would therefore likely be missed in current submillimeter surveys.
